PCL: Peer-Contrastive Learning with Diverse Augmentations for Unsupervised Sentence Embeddings

Learning sentence embeddings in an unsupervised manner is fundamental in natural language processing. Recent common practice is to couple pre-trained language models with unsupervised contrastive learning, whose success relies on augmenting a sentence with a semantically-close positive instance to construct contrastive pairs. Nonetheless, existing approaches usually depend on a mono-augmenting strategy, which causes learning shortcuts towards the augmenting biases and thus corrupts the quality of sentence embeddings. A straightforward solution is resorting to more diverse positives from a multi-augmenting strategy, while an open question remains about how to unsupervisedly learn from the diverse positives but with uneven augmenting qualities in the text field. As one answer, we propose a novel Peer-Contrastive Learning (PCL) with diverse augmentations. PCL constructs diverse contrastive positives and negatives at the group level for unsupervised sentence embeddings. PCL performs peer-positive contrast as well as peer-network cooperation, which offers an inherent anti-bias ability and an effective way to learn from diverse augmentations. Experiments on STS benchmarks verify the effectiveness of PCL against its competitors in unsupervised sentence embeddings.

==> 5-discussion.tex <==
Extensive empirical results have shown the effectiveness of PCL, but we still need to elaborate a couple of issues in this work and for future research of unsupervised sentence embeddings using contrastive learning.

\paragraph{How to choose augmentation strategies?}
As introduced in the section~\ref{sec:augs}, we manually choose five widely used augmentation strategies for texts. As the main goal of this paper is to verify the effectiveness of our PCL framework, all of the chosen augmentations are common and simple. We speculate that our PCL can be further improved with more fine-tuned augmentation strategies. We have presented that the number and diversity are both crucial to contrastive learning with multiple augmentation. Thus we suggest guaranteeing the diversity (i.e. augmenting texts from diverse perspectives) of chosen augmentations, and constructing at least five strategies to ensure the effectiveness of the framework.

\paragraph{Contrastive instances with multiple augmentations can be more noisy.}
Note that whether we use multiple augmentations or not, noisy positives are inevitable with uneven augmenting qualities in the text field. For example, given a sentence \textit{``A dog is chasing a cat.''}, possible bad positive instances are shown in the table~\ref{tab:augs}.
\input{tables/augs}
Constructing multiple positive instances may aggravate this issue.
% We define the \textit{noisy degree} of a training sample as the percentage of bad positive instances among all positive instances.
We can assume the possibility that a single augmentation strategy gives a bad positive instance is $p$. The possibility that there is at least one bad positive instance among $K$ positive instances is $p_m = 1-(1-p)^K$. Even assuming that $p$ is 0.1, the $p_m$ can be as large as 0.4 and 0.6 when $K$ is 5 and 9, respectively. Thus, and necessarily, our PCL propose co-operative learning objective, which offers a robust way to learn from noisy contrastive instances. Ablation study in the table~\ref{tab:ablation} shows that the performance of PCL drops by 1.02 without the co-operative learning objective, which also supports the necessity of learning from noises with multiple augmentations.

\paragraph{Apply PCL to supervised learning of sentence embeddings?}
We propose peer contrastive learning with diverse augmentations because unsupervised contrastive learning of sentence embedding is likely biased towards positive instance by mono-augmenting strategy. But supervised contrastive pairs are constructed from a more general semantic perspective, e.g. entailment or paraphrase. In contrast to unsupervised augmentation, it is hardly biased towards a particular semantic aspects (e.g. ordering, bag-of-words or sentence length), and also not noisy. Besides, such supervised datasets are scarce and require much human effort to collect, especially for minor language community~\cite{coulombe2018text}. Based on the discussion above and preliminary experiments, we focus on improving unsupervised sentence embeddings in this paper.

\paragraph{Are regularization approaches (e.g. dropout) biased?}
There are existing works utilize regularization methods, instead of text augmentation, to construct contrastive pairs. Take dropout as an 
example, SimCSE~\citet{gao2021simcse} constructs contrastive pairs by passing a single sentence into the encoder twice and obtain two different instances in embedding-level. Although it avoid generating false-positive instances, it may also make trivial contrastive pairs as the length of sentence is always the same. \citet{Wu2021ESimCSEES} also report that the performance of SimCSE gets worse when as the length difference of test pairs increases. Hence, the advantage of PCL maintains the advantage over approaches using mono-augmenting strategy, regardless if it is text augmentation or regularization. Experimental results in the table~\ref{tab:main_sts} and figure~\ref{fig:ablation_diversity} also support our standpoint.

==> images/ablation.tex <==
\begin{tikzpicture}
    \begin{axis}[
        width=\linewidth,
        height=.7\linewidth,
        ybar,
        % ymin=73.8,
        enlarge x limits =0.1,
        legend pos=north west,
        bar width=0.15cm,
        % bar shift=0pt,
        ylabel=Spearman's correlation,
        ylabel near ticks,
        xlabel near ticks,
        xticklabel style={rotate=45},
        xtick align=inside,
        font=\fontsize{9}{9}\selectfont, legend columns=3,
        legend style={
                at={(0.5, 1.2)},
                anchor=north
            },
        symbolic x coords={
            STS12, STS13, STS14, STS15, STS16, STSb, SICK-R, Avg.
        },
        xtick={STS12, STS13, STS14, STS15, STS16, STSb, SICK-R, Avg.},
        ytick={70,72.5,75,77.5,80,82.5},
        % nodes near coords,
        % nodes near coords style={above},
        point meta=y,
        grid=major,
    ]
    \addplot[draw=black, fill=MYRED][error bars/.cd,y dir=both, y explicit] coordinates {
        (STS12, 72.74) +- (0.58,-0.58)
        (STS13, 83.36) +- (0.40,-0.40) 
        (STS14, 76.05) +- (0.39,-0.39)
        (STS15, 83.07) +- (0.40,-0.40)
        (STS16, 79.26) +- (0.15,-0.15)
        (STSb, 79.72) +- (0.53,-0.53)
        (SICK-R, 72.75) +- (0.50,-0.50)
        (Avg., 78.14) +- (0.16,-0.16)
        };
    \addplot[draw=black, fill=MYBLUE][error bars/.cd,y dir=both, y explicit] coordinates {
        (STS12, 71.15) +- (0.93,-0.93)
        (STS13, 83.07) +- (0.55,-0.55) 
        (STS14, 75.72) +- (0.48,-0.48)
        (STS15, 82.93) +- (0.61,-0.61)
        (STS16, 78.37) +- (0.58,-0.58)
        (STSb, 78.67) +- (0.53,-0.53)
        (SICK-R, 70.37) +- (1.1,-1.1)
        (Avg., 77.18) +- (0.22,-0.22)
        };
    \addplot[draw=black, fill=MYORANGE][error bars/.cd,y dir=both, y explicit] coordinates {
        (STS12, 72.22) +- (0.62,-0.62)
        (STS13, 81.31) +- (0.47,-0.47) 
        (STS14, 74.34) +- (0.46,-0.46)
        (STS15, 82.39) +- (0.29,-0.29)
        (STS16, 79.51) +- (0.31,-0.31)
        (STSb, 79.27) +- (0.51,-0.51)
        (SICK-R, 71.93) +- (0.08,-0.08)
        (Avg., 77.28) +- (0.19,-0.19)
        };
    \addlegendentry{PCL}
    \addlegendentry{PCL$_{w/o D}$}
    \addlegendentry{PCL$_{w/o C}$}
    \end{axis}
\end{tikzpicture}

==> tables/augs.tex <==
\begin{table}[!t]
\centering
\small
\begin{tabular}{cc}
\toprule
Augmentation                          & Possible bad positive instances.              \\
\midrule
Shuffled Sentence                     & \textit{A cat is chasing a dog.}     \\ \midrule
Inversed Sentence                     & \textit{Dog a chasing is cat a.}     \\\midrule
Word Repetition & \textit{A dog is chasing a cat dog.} \\ \midrule
Word Deletion   & \textit{A is chasing a cat.}         \\ \bottomrule
\end{tabular}
\caption{Possible bad positive instances of text augmentations for a given example \textit{``A dog is chasing a cat.''}.}
\label{tab:augs}
\end{table}

==> tables/fix.tex <==
\begin{table}[!htbp]
\begin{tabular}{|c||c|c|}
\hline
Tasks  & PCL           & PCL$_{FixP}$    \\ \hline
STS12  & \textbf{72.74} & 70.65                       \\ \hline
STS13  & \textbf{83.36}          & 77.49              \\ \hline
STS14  & \textbf{76.05}          & 71.69              \\ \hline
STS15  & \textbf{83.07} & 79.45                      \\ \hline
STS16  & 79.26          & 78.87            \\ \hline
STSb   & \textbf{79.72} & 76.55                      \\ \hline
SICK-R & \textbf{72.75} & 72.46                       \\ \hline
Avg.   & \textbf{78.14} & 75.31                       \\ \hline
\end{tabular}
\caption{Ablation study on whether updating the extra peer encoder.}
\label{tab:fix}
\end{table}
